The Galaxy-Halo Connection Over The Last 13.3 Gyrs

We present new determinations of the stellar-to-halo mass relation (SHMR) at $z=0-10$ that match the evolution of the galaxy stellar mass function, the SFR$-M_*$ relation,and the cosmic star formation rate. We utilize a compilation of 40 observational studies from the literature and correct them for potential biases. Using our robust determinations of halo mass assembly and the SHMR, we infer star formation histories, merger rates, and structural properties for average galaxies, combining star-forming and quenched galaxies. Our main findings: (1) The halo mass $M_{50}$ above which 50\% of galaxies are quenched coincides with sSFR/sMAR$\sim1$, where sMAR is the specific halo mass accretion rate. (2) $M_{50}$ increases with redshift, presumably due to cold streams being more efficient at high redshift while virial shocks and AGN feedback become more relevant at lower redshifts. (3) The ratio sSFR/sMAR has a peak value, which occurs around $M_{\rm vir}\sim2\times10^{11}M_{\odot}$. (4) The stellar mass density within 1 kpc, $\Sigma_1$, is a good indicator of the galactic global sSFR. (5) Galaxies are statistically quenched after they reach a maximum in $\Sigma_1$, consistent with theoretical expectations of the gas compaction model; this maximum depends on redshift. (6) In-situ star formation is responsible for most galactic stellar mass growth, especially for lower-mass galaxies. (7) Galaxies grow inside out. The marked change in the slope of the size--mass relation when galaxies became quenched, from $d\log R_{\rm eff}/d\log M_*\sim0.35$ to $\sim2.5$, could be the result of dry minor mergers.

==> ExtraBibs.tex <==
\footnote{Here $M_{\mathcal{C}}(z)$ is the characteristic mass of halos just collapsing at redshift $z$. For the cosmological parameters used here, $M_{\mathcal{C}}(z)$ is given by Equation (31) and Figure 9 of \citet{Rodriguez-Puebla+2016}.}

@ARTICLE{Somerville+2015,
   author = {{Somerville}, R.~S. and {Dav{\'e}}, R.},
    title = "{Physical Models of Galaxy Formation in a Cosmological Framework}",
  journal = {\araa},
archivePrefix = "arXiv",
   eprint = {1412.2712},
     year = 2015,
    month = aug,
   volume = 53,
    pages = {51-113},
      doi = {10.1146/annurev-astro-082812-140951},
   adsurl = {http://adsabs.harvard.edu/abs/2015ARA%26A..53...51S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Bouwens+2011,
   author = {{Bouwens}, R.~J. and {Illingworth}, G.~D. and {Oesch}, P.~A. and 
	{Labb{\'e}}, I. and {Trenti}, M. and {van Dokkum}, P. and {Franx}, M. and 
	{Stiavelli}, M. and {Carollo}, C.~M. and {Magee}, D. and {Gonzalez}, V.
	},
    title = "{Ultraviolet Luminosity Functions from 132 z \~{} 7 and z \~{} 8 Lyman-break Galaxies in the Ultra-deep HUDF09 and Wide-area Early Release Science WFC3/IR Observations}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1006.4360},
 keywords = {galaxies: evolution, galaxies: high-redshift},
     year = 2011,
    month = aug,
   volume = 737,
      eid = {90},
    pages = {90},
      doi = {10.1088/0004-637X/737/2/90},
   adsurl = {http://adsabs.harvard.edu/abs/2011ApJ...737...90B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Salmon+2015,
   author = {{Salmon}, B. and {Papovich}, C. and {Finkelstein}, S.~L. and 
	{Tilvi}, V. and {Finlator}, K. and {Behroozi}, P. and {Dahlen}, T. and 
	{Dav{\'e}}, R. and {Dekel}, A. and {Dickinson}, M. and {Ferguson}, H.~C. and 
	{Giavalisco}, M. and {Long}, J. and {Lu}, Y. and {Mobasher}, B. and 
	{Reddy}, N. and {Somerville}, R.~S. and {Wechsler}, R.~H.},
    title = "{The Relation between Star Formation Rate and Stellar Mass for Galaxies at 3.5 {\lt}= z {\lt}= 6.5 in CANDELS}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1407.6012},
 keywords = {galaxies: distances and redshifts, galaxies: evolution, galaxies: fundamental parameters, Magellanic Clouds },
     year = 2015,
    month = feb,
   volume = 799,
      eid = {183},
    pages = {183},
      doi = {10.1088/0004-637X/799/2/183},
   adsurl = {http://adsabs.harvard.edu/abs/2015ApJ...799..183S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Noeske+2007,
   author = {{Noeske}, K.~G. and {Weiner}, B.~J. and {Faber}, S.~M. and {Papovich}, C. and 
	{Koo}, D.~C. and {Somerville}, R.~S. and {Bundy}, K. and {Conselice}, C.~J. and 
	{Newman}, J.~A. and {Schiminovich}, D. and {Le Floc'h}, E. and 
	{Coil}, A.~L. and {Rieke}, G.~H. and {Lotz}, J.~M. and {Primack}, J.~R. and 
	{Barmby}, P. and {Cooper}, M.~C. and {Davis}, M. and {Ellis}, R.~S. and 
	{Fazio}, G.~G. and {Guhathakurta}, P. and {Huang}, J. and {Kassin}, S.~A. and 
	{Martin}, D.~C. and {Phillips}, A.~C. and {Rich}, R.~M. and 
	{Small}, T.~A. and {Willmer}, C.~N.~A. and {Wilson}, G.},
    title = "{Star Formation in AEGIS Field Galaxies since z=1.1: The Dominance of Gradually Declining Star Formation, and the Main Sequence of Star-forming Galaxies}",
  journal = {\apjl},
   eprint = {astro-ph/0701924},
 keywords = {Galaxies: Evolution, Galaxies: Formation, Galaxies: High-Redshift, Galaxies: Starburst},
     year = 2007,
    month = may,
   volume = 660,
    pages = {L43-L46},
      doi = {10.1086/517926},
   adsurl = {http://adsabs.harvard.edu/abs/2007ApJ...660L..43N},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Blanton+2005a,
   author = {{Blanton}, M.~R. and {Lupton}, R.~H. and {Schlegel}, D.~J. and 
	{Strauss}, M.~A. and {Brinkmann}, J. and {Fukugita}, M. and 
	{Loveday}, J.},
    title = "{The Properties and Luminosity Function of Extremely Low Luminosity Galaxies}",
  journal = {\apj},
   eprint = {astro-ph/0410164},
 keywords = {Galaxies: Dwarf, Galaxies: Fundamental Parameters, Galaxies: Luminosity Function, Mass Function, Galaxies: Statistics},
     year = 2005,
    month = sep,
   volume = 631,
    pages = {208-230},
      doi = {10.1086/431416},
   adsurl = {http://adsabs.harvard.edu/abs/2005ApJ...631..208B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Chen+2009,
   author = {{Chen}, Y.-M. and {Wild}, V. and {Kauffmann}, G. and {Blaizot}, J. and 
	{Davis}, M. and {Noeske}, K. and {Wang}, J.-M. and {Willmer}, C.
	},
    title = "{Constraints on the star formation histories of galaxies from z \~{} 1 to 0}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {0808.3683},
 keywords = {galaxies: evolution},
     year = 2009,
    month = feb,
   volume = 393,
    pages = {406-418},
      doi = {10.1111/j.1365-2966.2008.14247.x},
   adsurl = {http://adsabs.harvard.edu/abs/2009MNRAS.393..406C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Moster+2013,
   author = {{Moster}, B.~P. and {Naab}, T. and {White}, S.~D.~M.},
    title = "{Galactic star formation and accretion histories from matching galaxies to dark matter haloes}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1205.5807},
 primaryClass = "astro-ph.CO",
 keywords = {galaxies: evolution, galaxies: high-redshift, galaxies: statistics, galaxies: stellar content, cosmology: theory, dark matter},
     year = 2013,
    month = feb,
   volume = 428,
    pages = {3121-3138},
      doi = {10.1093/mnras/sts261},
   adsurl = {http://adsabs.harvard.edu/abs/2013MNRAS.428.3121M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Salim+2007,
   author = {{Salim}, S. and {Rich}, R.~M. and {Charlot}, S. and {Brinchmann}, J. and 
	{Johnson}, B.~D. and {Schiminovich}, D. and {Seibert}, M. and 
	{Mallery}, R. and {Heckman}, T.~M. and {Forster}, K. and {Friedman}, P.~G. and 
	{Martin}, D.~C. and {Morrissey}, P. and {Neff}, S.~G. and {Small}, T. and 
	{Wyder}, T.~K. and {Bianchi}, L. and {Donas}, J. and {Lee}, Y.-W. and 
	{Madore}, B.~F. and {Milliard}, B. and {Szalay}, A.~S. and {Welsh}, B.~Y. and 
	{Yi}, S.~K.},
    title = "{UV Star Formation Rates in the Local Universe}",
  journal = {\apjs},
archivePrefix = "arXiv",
   eprint = {0704.3611},
 keywords = {Galaxies: Active, Galaxies: Evolution, Galaxies: Fundamental Parameters, Surveys, Ultraviolet: Galaxies},
     year = 2007,
    month = dec,
   volume = 173,
    pages = {267-292},
      doi = {10.1086/519218},
   adsurl = {http://adsabs.harvard.edu/abs/2007ApJS..173..267S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Shen+2003,
   author = {{Shen}, S. and {Mo}, H.~J. and {White}, S.~D.~M. and {Blanton}, M.~R. and 
	{Kauffmann}, G. and {Voges}, W. and {Brinkmann}, J. and {Csabai}, I.
	},
    title = "{The size distribution of galaxies in the Sloan Digital Sky Survey}",
  journal = {\mnras},
   eprint = {astro-ph/0301527},
 keywords = {galaxies: formation, galaxies: fundamental parameters, galaxies: statistics, galaxies: structure},
     year = 2003,
    month = aug,
   volume = 343,
    pages = {978-994},
      doi = {10.1046/j.1365-8711.2003.06740.x},
   adsurl = {http://adsabs.harvard.edu/abs/2003MNRAS.343..978S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Zavala+2012,
   author = {{Zavala}, J. and {Avila-Reese}, V. and {Firmani}, C. and {Boylan-Kolchin}, M.
	},
    title = "{The growth of galactic bulges through mergers in {$\Lambda$} CDM haloes revisited - I. Present-day properties}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1204.0516},
 primaryClass = "astro-ph.CO",
 keywords = {galaxies: bulges, galaxies: evolution, galaxies: formation, galaxies: interactions, galaxies: structure},
     year = 2012,
    month = dec,
   volume = 427,
    pages = {1503-1516},
      doi = {10.1111/j.1365-2966.2012.22100.x},
   adsurl = {http://adsabs.harvard.edu/abs/2012MNRAS.427.1503Z},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Grogin+2011,
   author = {{Grogin}, N.~A. and {Kocevski}, D.~D. and {Faber}, S.~M. and 
	{Ferguson}, H.~C. and {Koekemoer}, A.~M. and {Riess}, A.~G. and 
	{Acquaviva}, V. and {Alexander}, D.~M. and {Almaini}, O. and 
	{Ashby}, M.~L.~N. and {Barden}, M. and {Bell}, E.~F. and {Bournaud}, F. and 
	{Brown}, T.~M. and {Caputi}, K.~I. and {Casertano}, S. and {Cassata}, P. and 
	{Castellano}, M. and {Challis}, P. and {Chary}, R.-R. and {Cheung}, E. and 
	{Cirasuolo}, M. and {Conselice}, C.~J. and {Roshan Cooray}, A. and 
	{Croton}, D.~J. and {Daddi}, E. and {Dahlen}, T. and {Dav{\'e}}, R. and 
	{de Mello}, D.~F. and {Dekel}, A. and {Dickinson}, M. and {Dolch}, T. and 
	{Donley}, J.~L. and {Dunlop}, J.~S. and {Dutton}, A.~A. and 
	{Elbaz}, D. and {Fazio}, G.~G. and {Filippenko}, A.~V. and {Finkelstein}, S.~L. and 
	{Fontana}, A. and {Gardner}, J.~P. and {Garnavich}, P.~M. and 
	{Gawiser}, E. and {Giavalisco}, M. and {Grazian}, A. and {Guo}, Y. and 
	{Hathi}, N.~P. and {H{\"a}ussler}, B. and {Hopkins}, P.~F. and 
	{Huang}, J.-S. and {Huang}, K.-H. and {Jha}, S.~W. and {Kartaltepe}, J.~S. and 
	{Kirshner}, R.~P. and {Koo}, D.~C. and {Lai}, K. and {Lee}, K.-S. and 
	{Li}, W. and {Lotz}, J.~M. and {Lucas}, R.~A. and {Madau}, P. and 
	{McCarthy}, P.~J. and {McGrath}, E.~J. and {McIntosh}, D.~H. and 
	{McLure}, R.~J. and {Mobasher}, B. and {Moustakas}, L.~A. and 
	{Mozena}, M. and {Nandra}, K. and {Newman}, J.~A. and {Niemi}, S.-M. and 
	{Noeske}, K.~G. and {Papovich}, C.~J. and {Pentericci}, L. and 
	{Pope}, A. and {Primack}, J.~R. and {Rajan}, A. and {Ravindranath}, S. and 
	{Reddy}, N.~A. and {Renzini}, A. and {Rix}, H.-W. and {Robaina}, A.~R. and 
	{Rodney}, S.~A. and {Rosario}, D.~J. and {Rosati}, P. and {Salimbeni}, S. and 
	{Scarlata}, C. and {Siana}, B. and {Simard}, L. and {Smidt}, J. and 
	{Somerville}, R.~S. and {Spinrad}, H. and {Straughn}, A.~N. and 
	{Strolger}, L.-G. and {Telford}, O. and {Teplitz}, H.~I. and 
	{Trump}, J.~R. and {van der Wel}, A. and {Villforth}, C. and 
	{Wechsler}, R.~H. and {Weiner}, B.~J. and {Wiklind}, T. and 
	{Wild}, V. and {Wilson}, G. and {Wuyts}, S. and {Yan}, H.-J. and 
	{Yun}, M.~S.},
    title = "{CANDELS: The Cosmic Assembly Near-infrared Deep Extragalactic Legacy Survey}",
  journal = {\apjs},
archivePrefix = "arXiv",
   eprint = {1105.3753},
 primaryClass = "astro-ph.CO",
 keywords = {cosmology: observations, galaxies: high-redshift},
     year = 2011,
    month = dec,
   volume = 197,
      eid = {35},
    pages = {35},
      doi = {10.1088/0067-0049/197/2/35},
   adsurl = {http://adsabs.harvard.edu/abs/2011ApJS..197...35G},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Bouche+2010,
   author = {{Bouch{\'e}}, N. and {Dekel}, A. and {Genzel}, R. and {Genel}, S. and 
	{Cresci}, G. and {F{\"o}rster Schreiber}, N.~M. and {Shapiro}, K.~L. and 
	{Davies}, R.~I. and {Tacconi}, L.},
    title = "{The Impact of Cold Gas Accretion Above a Mass Floor on Galaxy Scaling Relations}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {0912.1858},
 keywords = {cosmology: observations, galaxies: evolution, galaxies: high-redshift},
     year = 2010,
    month = aug,
   volume = 718,
    pages = {1001-1018},
      doi = {10.1088/0004-637X/718/2/1001},
   adsurl = {http://adsabs.harvard.edu/abs/2010ApJ...718.1001B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Bundy+2009,
   author = {{Bundy}, K. and {Fukugita}, M. and {Ellis}, R.~S. and {Targett}, T.~A. and 
	{Belli}, S. and {Kodama}, T.},
    title = "{The Greater Impact of Mergers on the Growth of Massive Galaxies: Implications for Mass Assembly and Evolution since z sime 1}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {0902.1188},
 primaryClass = "astro-ph.CO",
 keywords = {galaxies: evolution, galaxies: formation, galaxies: interactions},
     year = 2009,
    month = jun,
   volume = 697,
    pages = {1369-1383},
      doi = {10.1088/0004-637X/697/2/1369},
   adsurl = {http://adsabs.harvard.edu/abs/2009ApJ...697.1369B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Mendel+2014,
   author = {{Mendel}, J.~T. and {Simard}, L. and {Palmer}, M. and {Ellison}, S.~L. and 
	{Patton}, D.~R.},
    title = "{A Catalog of Bulge, Disk, and Total Stellar Mass Estimates for the Sloan Digital Sky Survey}",
  journal = {\apjs},
archivePrefix = "arXiv",
   eprint = {1310.8304},
 primaryClass = "astro-ph.CO",
 keywords = {galaxies: bulges, galaxies: fundamental parameters, galaxies: statistics, galaxies: structure },
     year = 2014,
    month = jan,
   volume = 210,
      eid = {3},
    pages = {3},
      doi = {10.1088/0067-0049/210/1/3},
   adsurl = {http://adsabs.harvard.edu/abs/2014ApJS..210....3M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Dave+2012,
   author = {{Dav{\'e}}, R. and {Finlator}, K. and {Oppenheimer}, B.~D.},
    title = "{An analytic model for the evolution of the stellar, gas and metal content of galaxies}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1108.0426},
 keywords = {galaxies: evolution, galaxies: formation, galaxies: fundamental parameters, galaxies: haloes, galaxies: high-redshift, intergalactic medium},
     year = 2012,
    month = mar,
   volume = 421,
    pages = {98-107},
      doi = {10.1111/j.1365-2966.2011.20148.x},
   adsurl = {http://adsabs.harvard.edu/abs/2012MNRAS.421...98D},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}
@ARTICLE{Krumholz+2012,
   author = {{Krumholz}, M.~R. and {Dekel}, A.},
    title = "{Metallicity-dependent Quenching of Star Formation at High Redshift in Small Galaxies}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1106.0301},
 keywords = {cosmology: theory, galaxies: formation, galaxies: high-redshift, galaxies: ISM, ISM: molecules, stars: formation},
     year = 2012,
    month = jul,
   volume = 753,
      eid = {16},
    pages = {16},
      doi = {10.1088/0004-637X/753/1/16},
   adsurl = {http://adsabs.harvard.edu/abs/2012ApJ...753...16K},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Dekel+2013,
   author = {{Dekel}, A. and {Zolotov}, A. and {Tweed}, D. and {Cacciato}, M. and 
	{Ceverino}, D. and {Primack}, J.~R.},
    title = "{Toy models for galaxy formation versus simulations}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1303.3009},
 keywords = {galaxies: evolution, galaxies: formation, galaxies: haloes, dark matter},
     year = 2013,
    month = oct,
   volume = 435,
    pages = {999-1019},
      doi = {10.1093/mnras/stt1338},
   adsurl = {http://adsabs.harvard.edu/abs/2013MNRAS.435..999D},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

